On Coreferring Text-extracted Event Descriptions with the aid of Ontological Reasoning

Systems for automatic extraction of semantic information about events from large textual resources are now available: these tools are capable to generate RDF datasets about text extracted events and this knowledge can be used to reason over the recognized events. On the other hand, text based tasks for event recognition, as for example event coreference (i.e. recognizing whether two textual descriptions refer to the same event), do not take into account ontological information of the extracted events in their process. In this paper, we propose a method to derive event coreference on text extracted event data using semantic based rule reasoning. We demonstrate our method considering a limited (yet representative) set of event types: we introduce a formal analysis on their ontological properties and, on the base of this, we define a set of coreference criteria. We then implement these criteria as RDF-based reasoning rules to be applied on text extracted event data. We evaluate the effectiveness of our approach over a standard coreference benchmark dataset.

==> sec/model.tex <==
\section{Formalizing and reasoning about events}

The literature offers many logical formalisms for 
representing logically events and reasoning about them. 
Situation calculus, Event calculus, logic of context, action logics,
\dots. When information are represented in RDF format on the basis of
OWL ontoloties one can choose different schemata, depending on the
the adopted formalization. A detailed comparison on the schema used to
represent time dependent information in RDF and OWL can be found in 
\cite{annotation-time-dependent-knowledge-in-sw-krieger2014}. 

\subsection{Formal description of events} 

\todo{Come formalizziamo gli eventi noi} 

\subsection{Reasoning about Events (Loris + Luciano)}
\lbnote{Old stuff: aggiornare con modello e regole necessarie per coreference}

{\color{red} using the CKR framework to represent events. }

{\color{red} What are the correct inferences on events? Add here a set
  of infrerences about event informaiton, which we conider to be
  general and sound} 

We don't suppose here to give an exhaustive list of the sound
inferences about evnet knowledge. This will be the subject of 
a future work. We, instead, provide a set of rule which are strong
enough to infer interesting, unknown, facts which are relevant to the
scenarios that we have described in the introduction. 

